Magnetic Fields in Blazar Pc-scale Jets - Possible connection to Spin Rates of Black holes ?

We re-examine the differences observed in the pc-scale magnetic field geometry of high and low optical polarization Quasars (HPQs, LPRQs) using the MOJAVE sample. We find that, as previously reported, HPQ jets exhibit predominantly transverse B fields while LPRQ jets tend to display longitudinal B fields. We attempt to understand these results along with the different B field geometry observed in the low and high energy peaked BL Lacs (LBLs, HBLs) using a simple picture wherein the spinning central black holes in these AGNs influence the speed and strength of the jet components (spine, sheath). Higher spin rates in HPQs compared to LPRQs and LBLs compared to HBLs could explain the different total radio powers, VLBI jet speeds, and the observed B field geometry in these AGN classes.

==> RESPONSE <==

We thank the referee for a careful reading of our manuscript and
suggesting changes that have improved the paper. We have incorporated
all the suggested changes. Our response is marked below as 1A, 2A, etc.

===========================================================================

1. The authors use "LPRQ" as abbreviation for "low optical polarization 
radio quasars". Is there a specific reason for this use instead of the 
more common abbreviation "LPQ"? Otherwise, I suggest to use "LPQ" instead 
of "LPRQ".
----------------------------------------------------------------------------
1A. The term "LPRQ" was used by Lister & Smith (2000)[ApJ.541.66] to 
refer to radio-loud quasars so as to differentiate them from the radio-quiet 
variety, which could also have low optical polarization. The high 
polarization quasars, on the other hand, are invariably radio-loud.
We have therefore retained the use of the terms "LPRQ" and "HPQs".
----------------------------------------------------------------------------

2. I suggest to
- change "blackhole" to "black hole" throughout the paper (title,
   abstract, main text)
- change "magnetic-field" (abstract, l.1; conclusions, l.1) to "magnetic
   field"
- change "homogenous" (introduction, l.11) to "homogeneous"
- add "Meier [9]..." before reference [9] in 3.1., l.1.
- change "jet acceleration" to "flow acceleration" on p.3, l. 5.
- change "plausible" to "possible" in the last line in 3.1., as some of
   the theoretical scenarios mentioned before in 3.1. rather seem to
   suggest the opposite.
----------------------------------------------------------------------------
2A. All the above suggested changes have been made in the paper.
----------------------------------------------------------------------------

3. I suggest to introduce/define $\theta_{\rm jet}$ and $chi$ (Fig.1) in 
the caption of Fig. 1, e.g., "EVPAs $\chi_{\rm jet} w.r.t. the VLBI jet 
direction $\theta$..."
----------------------------------------------------------------------------
3A. This is now done.
----------------------------------------------------------------------------

4. By spine dominance (e.g., "However, the spine dominates in the highest 
spin rate HPQs...", p.3) do the authors mean dominance of its magnetic 
field (strength etc.) or just the relative width spine/sheath (I suppose 
the latter). Adding a short clarification may be useful.
----------------------------------------------------------------------------
4A.  We have added a small paragraph (Para 2) in Section 3.1, Page 3, to 
make our statements clearer.
----------------------------------------------------------------------------

5. Is there a simple physical reason why the magnetic field in the spine 
should be transverse? If so, it may be worth adding a short line...
----------------------------------------------------------------------------
5A. We have now added a few explanatory sentences in Para 1, Section 3.1, 
Page 3, about the B field structure and added two new references - 
Meier et al. (2001) and Laing (1981). 
----------------------------------------------------------------------------

6. References:
- page number is missing in reference for R. Laing
- Ghisellini et al.: change "AAP" to "A\&A"
----------------------------------------------------------------------------
6A. This is now taken care of.
===========================================================================

In addition to the changes suggested by the referee, we have made a 
few changes. These include -

1. In Section 3, we have added a new short paragraph (Para 3) mentioning the 
need for getting extended emission data for these sources and our ongoing 
project to obtain them.

2. In Section 3.2, we have removed the third paragraph and Figure 5. 
This is because of realising that this plot and result is likely to be 
strongly affected by variability. We are in the process of estimating the 
radio core prominence from simultaneously acquired core and extended 
emission data. This will form part of a future paper.

3. In Section 3.2, we have added a new small second paragraph about Radio 
core power. 

A few minor textual changes have been made throughout to improve the 
readability of the paper.

